Timing-driven Approximate Logic Synthesis Based on Double-chase Grey Wolf Optimizer

With the shrinking technology nodes, timing optimization becomes increasingly challenging. Approximate logic synthesis (ALS) can perform local approximate changes (LACs) on circuits to optimize timing with the cost of slight inaccuracy. However, existing ALS methods that focus solely on critical path depth reduction (depth-driven methods) or area minimization (area-driven methods) are inefficient in achieving optimal timing improvement. %based on double-chase grey wolf optimizer (DCGWO). where we employ a double-chase grey wolf optimizer to explore and apply LACs, simultaneously bringing excellent critical path shortening and area reduction under error constraints. According to experiments on open-source circuits with TSMC 28nm technology, compared to the SOTA method, our framework can generate approximate circuits with greater critical path delay reduction under different error and area constraints.

==> Makefile <==
ENGINE := pdflatex
BIB := bibtex

PROJECT := DATE25-SizingALS

all:
	$(ENGINE) $(PROJECT).tex
	$(BIB)    $(PROJECT)
	$(BIB)    $(PROJECT)
	$(ENGINE) $(PROJECT).tex
	$(ENGINE) $(PROJECT).tex

fast:
	$(ENGINE) $(PROJECT).tex


clean:
	rm -rf *.log *.aux *.blg *.bbl *.gz *.dvi *.thm *.dat *.out *latexmk *fls *busy\)



==> abstract.tex <==
\begin{abstract}
With the shrinking technology nodes, timing optimization becomes increasingly challenging.
Approximate logic synthesis (ALS) can perform local approximate changes (LACs) on circuits to optimize timing with the cost of slight inaccuracy.
However, existing ALS methods that focus solely on critical path depth reduction (depth-driven methods) or area minimization (area-driven methods) are inefficient in achieving optimal timing improvement.
%Meanwhile, constructing effective ALS methods targeting both critical path depth and area remains tricky due to the dispersion of optimization gradients.
In this work, we propose an effective timing-driven ALS framework,
%based on double-chase grey wolf optimizer (DCGWO).
where we employ a double-chase grey wolf optimizer to explore and apply LACs, simultaneously bringing excellent critical path shortening and area reduction under error constraints.
%The framework employs DCGWO to simultaneously shorten critical path and reduce area under error constraints.
Subsequently, it utilizes post-optimization under area constraints to convert area reduction into further timing improvement, thus achieving maximum critical path delay reduction.
%Based on experiments using open-source circuits with TSMC 28nm technology, our framework can generate approximate circuits with optimal critical path delay reduction under different error and area constraints.
According to experiments on open-source circuits with TSMC 28nm technology, compared to the SOTA method, our framework can generate approximate circuits with greater critical path delay reduction under different error and area constraints.
%for random/control circuits, our framework achieves an average $27.13\%$ critical path delay reduction under a $5\%$ error rate constraint; for arithmetic circuits, our framework achieves an average $38.54\%$ critical path delay reduction under a $2.44\%$ normalized mean error distance constraint, both of which outperform the state-of-the-art.
\end{abstract}



==> doc/DCGWO.tex <==
\section{Proposed Framework}
\label{Optimizer Overflow}
The overall flow of our proposed framework is given in \Cref{Overflow}.
In step \textcircled{\footnotesize{$1$}}, the accurate gate-level netlist is represented by gate fan-in adjacency lists.
In step \textcircled{\footnotesize{$2$}}, double-chase grey wolf optimizer (DCGWO) simultaneously optimizes critical path depth and area under error constraints.
%conducts multi-objective optimization targeting both timing and area under error constraints.
It can efficiently search for optimal approximate circuit through iterative circuit optimization, evaluation and circuit population update. 
%First, we initialize a population containing a large number of approximate circuits through LACs, and calculate fitness of each circuit.
%Next, we use the double-chase-based circuit optimization on the population to obtain approximate circuit candidates.
%Their fitness and errors are derived through circuit evaluation.
%Subsequently, We use non-dominated circuit sorting to select excellent approximate circuits from the candidates group and relax the error constraint asymptotically for circuit optimization in next iteration, until the iteration limit $I_{max}$ is reached.
In step \textcircled{\footnotesize{$3$}}, by performing dangling gates deletion and remaining gates sizing under area constraint $\text{Area}_{con}$ on the generated optimal approximate circuit, the final approximate netlist with maximum critical path delay reduction can be obtained.
% Overflow

% figure end 

\subsection{Circuit Representation}
\label{CR}
%In circuit netlists that use only single-output standard cells, each wire is connected to the output of exactly one gate.
%Circuit netlists are composed of single-output standard cells.
%In circuits, each wire is connected to the output of one gate.
%In circuit netlists, each wire is connected to the output of one gate.
%composed of single-output standard cells
%Therefore, we first analyze the wire-related information in the circuit netlist to obtain fan-in relationships between gates.
%Then, we construct adjacency lists that store the circuit structure based solely on these fan-in relationships.
We construct adjacency lists storing the circuit structure based solely on fan-in relationships between gates.
%By discarding all wire information, LACs and the generation of approximate netlists are accelerated.
By discarding all wire information, the LACs used in our framework, including wire-by-wire \cite{venkataramani2013substitute} and wire-by-constant \cite{schlachter2017design} replacements (shown in \Cref{gca}), can be easily implemented by changing the gate fan-in adjacency.
This operation mode enables us to efficiently assess the impact of LACs and generate corresponding approximate netlist.
%on the circuit structure
% By neglecting wires, LACs can be implemented simply, and the generation of approximate netlists is accelerated.
To check for circuit loop violations, we further label each gate with a unique integer ID.
%All gate-related information can be indexed using this ID.
\Cref{adj} shows an example of circuit representation, the circuit on the left is stored as fan-in adjacency lists on the right.
\iffalse
In addition, the order of the IDs helps us determine whether the generated approximate circuit contains any loop structures.
\fi

%Since we discard all wire information when storing the circuit structure, wire-by-wire and wire-by-constant replacements (introduced in \Cref{sec:model}) can be achieved by changing the fan-in adjacency of gates.
%This operation mode enables us to efficiently assess the impact of LACs on the circuit structure.
To accommodate this circuit representation method, we update the related definitions of above two LACs: the gate to be changed is called target gate, while the gate used for change (constant `0$/$1' are also treated as gates) is called switch gate.

\subsection{Double-chase Grey Wolf Optimizer}
\label{ACG}
In DCGWO, we first generate the initial approximate circuits population $\mathcal{P}_{0}$: $\{ \forall c_i \in \mathcal{P}_{0}\}$ by performing LACs on randomly selected target gates of the accurate circuit.
%Specifically, it involves performing LACs on randomly selected target gates of the accurate circuit to generate an initial population of approximate circuits $\mathcal{P}_{0}$: $\{ \forall c_i \in \mathcal{P}_{0}\}$.
Each approximate circuit in $\mathcal{P}_{0}$ is evaluated for fitness (defined in \cref{fitness} as function $Fit$), which is composed of critical path depth and area.
Circuits with higher fitness values indicate better quality. %Since the calculation of fitness involves some subsequent operations, its detailed definition will be provided in \cref{fitness}.
%The initial population participates in iterative optimization.

\minisection{Circuit Optimization}
As shown in \Cref{Overflow}, in each iteration, we perform the double-chase strategy to optimize approximate circuits in the population.
%(i.e., initial population or new population generated by population update in the previous iteration).
The preliminary work for double-chase involves the population division shown in \Cref{population division}.
It divides the population into leader circuit $c_l$, elite circuits $\mathcal{G}_{e}$, and $\omega$ circuits group $\mathcal{G}_\omega$ based on their fitness values.
Specifically, the leader circuit $c_l$ is the approximate circuit with the highest fitness.
%in the circuit population.
It guides the elite circuits with fitness ranks 2, 3, and 4 in Chase 1.
The elite circuits guide $\omega$ circuits group in Chase 2.
For Chase 1 and 2, we design two approximate actions: \textbf{circuit searching} and \textbf{circuit reproduction}. They are used alternately to generate new approximate circuits along suitable optimization gradients.
% population division
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{adj3.pdf}
    \caption{Circuit representation based on gate fan-in adjacency.}
    \label{adj}
\vspace{0.4in}
\end{figure}

% figure end

%\noindent\textbf{Circuit Searching.} 
The circuit searching essentially uses wire-by-wire and wire-by-constant to shorten critical paths. 
% To achieve efficient timing optimization, we select target gates on the critical path during circuit searching.
Specifically, we first use PrimeTime \cite{primetime} to obtain the critical paths with maximum propagation time from primary input (PI) to primary output (PO).
Then, for each critical path, all gates on it are stored in the targets set $\mathcal{T}_c$ and undergo uniform (0,1) distribution sampling.
All fan-ins of sampled gates with a probability greater than 0.5 are also stored in $\mathcal{T}_c$.
%Then, we perform the uniform (0, 1) distribution sampling of all gates on the critical path. 
%All fan-ins of gates with a probability greater than 0.5, along with all gates on the critical path, form a set.
The target gate is randomly selected from $\mathcal{T}_c$.
%The selection method for switch gate is the same as described in \Cref{sec:model}, where the similarity between target wire and switch object is equivalent to the similarity between the outputs of target gate and switch gate.
To limit introduced error, switch gate is selected based on similarities, i.e., the percentage of cycles when output of target gate holds the same value with output of each gate in its transitive fan-in (TFI) or the constant logic value `0', `1'.
The gate or constant logic value with the highest similarity is selected to substitute the target gate.
%Note that for a circuit with multiple critical paths, LAC is applied to each critical path.

\Cref{ReP} shows circuit searching examples.
For obtaining $c_{s1}$ from $c_{p1}$ through wire-by-constant searching, Path1 is the critical path. Thus we select ID8 gate (outputs: 14 cycles of `0' and 2 cycles of `1') as the target gate, and constant logic value `0' with the highest similarity 0.875 as the switch gate.
%The result of this circuit searching is that 
In this case, the fan-in adjacency of the ID11 gate is changed from (5, 8) to (5, con0), greatly decreasing the Path1 depth.
Similarly, for obtaining $c_{s2}$ from $c_{p2}$, the fan-in adjacency of ID15 PO is changed from 12 to 10, decreasing the Path3 depth.
%by neglecting ID12 gate.
%since $Path3$ is the critical path, ID12 gate is selected as target gate, and switch gate is ID10 gate with the highest similarity.  by wire-by-wire searching

%\noindent\textbf{Circuit Reproduction.} 
Inspired by a crossover in genetic algorithm \cite{deb2002fast}, circuit reproduction is designed to aggregate well-optimized path sets with low errors from two selected approximate circuits, generating a reproduced circuit with better quality.
%aggregate excellent structures of different circuits into a single circuit.
%To aggregate excellent structures from different approximate circuits into one circuit, we also design the circuit reproduction.
Specifically, we first divide each selected circuit according to the POs and corresponding TFI.
Then, for each PO, we use its maximum arrival time $T_a$ and the error generated on it $Error$ to form the PO-TFI pair evaluation function $Level$ in \Cref{level_calc}, where $w_{\text {t}}$ and $w_{\text {e}}$ are the weights of $T_a$ and $Error$ respectively. 
%($w_{\text {d}}\gg w_{\text {e}}$).
\begin{equation}
Level(PO_i)=w_{\text {t}}\times \frac{1}{T_a(PO_i)} + 
w_{\text {e}}\times \frac{1}{Error(PO_i)}.
\label{level_calc}
\end{equation}

Subsequently, we choose PO-TFI pairs with higher $Level$ from two selected circuits to form the reproduced circuit.
Some gates are shared by different PO-TFI pairs. 
Thus, gates in the reproduced circuit only accept adjacency information from the first write-in.
Taking circuits $c_{p1}$ and $c_{p2}$ in \Cref{ReP} as an example, by comparing their $Level$, we select PO2-TFI, PO3-TFI pairs from $c_{p1}$, and PO1-TFI pair from $c_{p2}$, to form circuit $c_{r1}$.
Since gates with IDs 8, 10 and 12 are not in any PO-TFI pair, to ensure the completeness of $c_{r1}$, their information is selected from $c_{p1}$ and $c_{p2}$ to write in $c_{r1}$.
%During this process, gates with IDs 8, 10, 12 are dangling due to their inability to connect to any PO.


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{division.pdf}
    \caption{Population division. Population is divided into leader $c_l$, elite circuits $\mathcal{G}_{e}$, and $\omega$ circuits group $\mathcal{G}_\omega$ based on fitness, with each hierarchy engaging in distinct chase operations.}
    \label{population division}
\vspace{-0.04in}
\end{figure}
% figure end

% reproduction
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=1\linewidth]{doublechase1.pdf}
    \caption{Illustrations of the circuit searching, circuit reproduction, and optimization gradients guided by them in double-chase.}
    \label{ReP}
\vspace{-0.1in}
\end{figure*}

%\noindent\textbf{Double-chase Decision.} 
\Cref{population division} illustrates that approximate circuits at different hierarchies consult their adjacent higher-hierarchy circuits for circuit searching and reproduction.
Therefore, we design the fitness distance $D$, decision parameter $W$ and decision threshold $S$ for both elite circuits $\mathcal{G}_{e}$ and $\omega$ circuits group $\mathcal{G}_\omega$.
$D$ is calculated by \Cref{D}, where $r_c$ is defined as a random value between $[0,2]$.
Since $\mathcal{G}_{e}$ reference the leader circuit $c_l$ for Chase 1, $D$ for elite circuits in $\mathcal{G}_{e}$ include the fitness of leader circuit $Fit(c_l)$.
Similarly, $\mathcal{G}_\omega$ reference $\mathcal{G}_e$ for Chase 2.
Thus, $D$ for $\omega$ circuits in $\mathcal{G}_\omega$ include the average fitness of elite circuits in $\mathcal{G}_e$.
$W$ provides a dynamic correction to $D$ by adding the encircling coefficient $A$.
%, as defined in \Cref{W}.
\begin{align}
\label{D}
	D(c_i) =
	\begin{cases}
		r_c\times Fit(c_l)-Fit(c_i) \hfill \forall c_i\in \mathcal{G}_{e}\\
		\frac{r_c}{3} \sum_{c_j\in \mathcal{G}_e} Fit\left ( c_j \right )-Fit(c_i) \quad \hfill \forall c_i\in \mathcal{G}_{\omega}\\
	\end{cases},
\end{align}

\begin{equation}
W(c_i)=A\times D(c_i),
\label{W}
\end{equation}
where $A$ is calculated based on the scaling factor $a$ as:
\begin{equation}
A=(2\times r_1-1)\times a,
\label{A}
\end{equation}
where $r_1$ is a random value between $[0,1]$. 
%allowing the population to dynamically search for the optimal approximate solution.
The scaling factor $a$ balances the global search and local convergence of the population during the iterative process.
As shown in \Cref{a}, $a$ decreases with the increase of iteration $iter$ until $iter$ reaches the upper limit of iteration $I_{\max}$.
\begin{equation}
a=2-\frac{2\times iter}{I_{\max}}.
\label{a}
\end{equation}
%The encircling coefficient $A$ maps $a$ to the actual double-chase behavior.
%Its definition is shown in \Cref{A}, where $r_1$ is a random value between $[0,1]$, allowing the population to dynamically search for the optimal approximate solution.

%The encircling coefficient $A$ maps $a$ to the actual search and convergence behavior.
%Its definition is shown in \Cref{A}, where $r_1$ is a random value between $[0,1]$, allowing the population to dynamically search for the optimal approximate solution.


%The attraction coefficient $C$ is defined as a random value between $[0,2]$. It serves to enhance the randomness of the %search process, reducing the possibility of getting trapped in local optima.



%Corresponding to $\mathcal{G}_{e}$ and $\mathcal{G}_\omega$, the decision thresholds $S$ are respectively $S_e$ and $S_{\omega}$.
As shown in \Cref{population division}, the approximate actions are decided by the relationship between decision parameter $W$ and decision thresholds $S$. 
Decision thresholds used for $\mathcal{G}_{e}$ and $\mathcal{G}_\omega$ are $S_e$ and $S_{\omega}$, respectively.
For circuit $c_i$ in $\mathcal{G}_{e}$, if $W(c_i)>S_e$, it executes circuit reproduction with another circuit of superior fitness to generate a reproduced circuit.
Otherwise, it uses circuit searching to reduce its critical path depth and area.
%Meanwhile, for circuit $c_i$ in $\mathcal{G}_{\omega}$, if $W(c_i)>S_\omega$, it engages in the circuit searching, and has a probability $p_{re}$ to form a pair with another high-fitness circuit for the circuit reproduction.
Meanwhile, for circuit $c_i$ in $\mathcal{G}_{\omega}$, if $W(c_i)>S_\omega$, it performs both circuit searching and reproduction.
Otherwise, it randomly selects either circuit searching or reproduction.
When the double-chase is completed, the leader $c_l$ conducts circuit searching to ensure its variability.
Then, approximate circuits before and after double-chase are stored in the candidates' group $\mathcal{G}_{cand}$ for further evaluation and update. 
%new approximate circuits generated by double-chase, together with the old population, are stored in the candidates group $\mathcal{G}_{cand}$ for further evaluation.
%reducing the possibility of the population falling into local optima.

The lower right corner of \Cref{ReP} demonstrates that the double-chase strategy can effectively guide the entire population to move along the appropriate gradient with simultaneous critical path depth and area reductions.
%thereby achieving efficient optimization.

%The above double-chase process generates a large number of new approximate circuits. However, an excessively large population is inefficient for optimization. Therefore, these new circuits, together with the population before double-chase, form a candidates group $\mathcal{G}_{cand}$ that will undergo fitness evaluation and population update.

%\subsubsection{Internal and external archive interaction.}
%\quad In the double-chase process, to prevent error surges or delay degradation caused by inappropriate approximate operations, we establish an external archive $AR_{\text {ex}}$ and an internal archive $AR_{\text {in}}$ to store the historical or generational information of the population.
%$AR_{\text {ex}}$ stores the leader circuits generated during the iterations, interacting with the double-chase process in the population division phase.
%In each iteration, the leader circuit $c_{l}$ with fitness $F_{l}$ is compared with the circuit $c_{best}$ with the highest fitness $F_{max}$ in $AR_{\text {ex}}$. 
%If $F_{l} \ge F_{max}$, $c_{l}$ will be inserted into $AR_{\text {ex}}$.
%Otherwise, $c_{l}$ will be replaced by $c_{best}$.
%The internal archive $AR_{\text {in}}$ stores the population screened in previous iteration and the new approximate circuits generated during the double-chase process.
%The approximate circuits in $AR_{\text {in}}$ will undergo further simulation, fitness evaluation, and non-dominated sorting.

\minisection{Circuit Fitness Evaluation}
\label{fitness}
%Since our optimization targets both timing and area, 
The fitness function is composed of two optimization objectives: critical path depth and area.
%, effectively evaluating the quality of approximate circuits.
The depth-related information, including the maximum critical path depth of each approximate circuit $Depth_{\text{app}}$ and the depth of the longest path in corresponding accurate circuit $Depth_{\text{ori}}$, are obtained through static timing analysis using PrimeTime \cite{primetime}.
Since circuit searching and reproduction change the connection relationship between gates, some gates become dangling due to their inability to connect to any PO.
%Since circuit searching and reproduction change the gates connection relationship, some gates become dangling as they no longer participate in any path connecting to the PO.
Therefore, the area of each approximate circuit $Area_{\text{app}}$ is the area of accurate circuit $Area_{\text {ori}}$ minus the area of these dangling gates.
\iffalse
The approximate circuit area $Area_{\text{app}}$ changes due to circuit searching and reproduction.
To calculate it, we first introduce the concept of Max Fanout Free Cone (MFFC), a subset of the transitive fan-in (TFI).
When one gate is removed, all gates in its MFFC become dangling due to their inability to connect to any PO. 
In a reproduction operation, $Area_{\text{app}}$ of the reproduced circuit inherits the larger area of two circuits for reproduction.
In a searching operation, $Area_{\text{app}}$ of the searched circuit is calculated by \Cref{Area}, where $AREA_{\text {bs}}$ represents the circuit area before this searching operation.
\begin{equation}
AREA_{\text{app}}=AREA_{\text {bs}}-AREA_{\text {mffc}}.
\label{Area}
\end{equation}

For the area reduction $AREA_{\text {mffc}}$ in \Cref{Area}, if the switch gate is a constant, or not in the TFI of the target gate, $Area_{\text {mffc}}$ is the total area of gates in the MFFC of target gate.
If the switch gate is in the TFI of the target gate, $AREA_{\text {mffc}}$ is the total area of gates in the difference set between the MFFCs of the target gate and switch gate.
\fi

The fitness function $Fit$ of approximate circuit $c_i$ is defined in \Cref{fit_calc}, where $w_{\text {d}}$ and $w_{\text {a}}=1-w_{\text {d}}$ respectively denote the weights assigned to the critical path depth and area. 
%and $c_i\in$ $\mathcal{P}_{0}$ or $\mathcal{G}_{cand}$ (i.e., candidate circuits group generated by double-chase).
Circuits with higher fitness values indicate better quality.
\begin{equation}
Fit(c_i)=w_{\text {d}}\times \frac{Depth_{\text {ori}}(c_i)}{Depth_{\text {app}}(c_i)} + 
w_{\text {a}}\times \frac{Area_{\text {ori}}(c_i)}{Area_{\text {app}}(c_i)}.
\label{fit_calc}
\end{equation}

\minisection{Circuit Population Update}
\label{pu}
\iffalse
The circuit population update is divided into two stages: non-dominated circuit sorting, asymptotic error-bound relaxation.
\fi
To select high-quality approximate circuits under error constraints, we perform non-dominated sorting \cite{zhang2014efficient} on the evaluated candidates' group $\mathcal{G}_{cand}$.
%This operation is essentially a Pareto set partition based on Pareto dominance, and the dominance relationship between approximate circuits is determined by their delay, area and error.
It is achieved based on Pareto dominance between circuits determined by two functions: depth function $f_d=\frac{Depth_{\text {ori}}}{Depth_{\text {app}}}$ and area function $f_a=\frac{Area_{\text {ori}}}{Area_{\text {app}}}$.
Firstly, we remove circuits exceeding the specified error constraint from $\mathcal{G}_{cand}$. 
Then, we maintain the dominated list $\mathcal{L}_{\text{d}}$ for each remaining circuit. % which can be obtained by traversing $\mathcal{G}_{cand}$.
For approximate circuits $c_i$ and $c_j$,  if $c_i$ is not inferior to $c_j$ in two functions, and is superior in at least one of them, then $c_i$ dominates $c_j$ and is added to $\mathcal{L}_{\text{d}}$
of $c_j$.
Circuits with empty $\mathcal{L}_{\text{d}}$ are considered Pareto-optimal circuits. We place them into the 0-ranked Pareto set while removing them from $\mathcal{G}_{cand}$ and the $\mathcal{L}_{\text{d}}$ of other circuits.
%When an approximate circuit is not dominated by any other circuits (i.e., the $\mathcal{L}_{\text{d}}$ is empty), we call it a Pareto-optimal circuit.
%After obtaining the $\mathcal{L}_{\text{d}}$ for all approximate circuits, we place the initial Pareto-optimal circuits into the 0-ranked Pareto set while removing them from $\mathcal{G}_{cand}$ and the $\mathcal{L}_{\text{d}}$ of other circuits.
Subsequently, new Pareto-optimal circuits with empty $\mathcal{L}_{\text{d}}$ emerge, forming the 1-ranked Pareto set, and undergo the same removal process. 
This will repeat until $\mathcal{G}_{cand}$ is empty.
%It is noteworthy that approximate circuits exceeding the specified error constraint are moved to the violation set.
%This set serves as the highest-ranked Pareto set, indicating that all circuits with error violations are dominated by any other circuits.

%As for population update, if the approximate circuits retained after each update are relatively dispersed in the objective function space, the approximate solutions generated after the double-chase are less likely to overlap, resulting in higher search efficiency. 
We further calculate the crowding distance $Dist$ of approximate circuits in each Pareto set.
With higher $Dist$, circuits are less likely to overlap in the objective function space, resulting in better optimization efficiency.
%In the $k$-ranked Pareto set, the objective functions for each approximate circuit are $f_d=CPD_{\text{app}}$ and $f_a=AREA_{\text{app}}$.
%which are equivalent to its critical path delay $CPD_{\text{app}}$ and area $AREA_{\text{app}}$. 
%Before calculating the $Dist$, 
%We sort the circuits in this Pareto set based on $f_d$ and $f_a$ separately.
In the $k$-ranked Pareto set, approximate circuits are sorted separately based on $f_d$ and $f_a$.
The $Dist$ of the circuits at the beginning and end of these two sorted lists are set to $+\infty$.
For approximate circuit $c_i$, circuits adjacent to $c_i$ in each sorted list are $c_{i-1}$ and $c_{i+1}$.
In this case, $Dist$ is calculated by \Cref{D_crowd}.
%where $max(f_j)$ and $min(f_j)$ refer to the maximum and minimum objective function values in the $i$-ranked Pareto set, respectively.
\begin{equation}
Dist(c_i)=\sum_{x=d,a}\frac{f_x(c_{i-1})-f_x{(c_{i+1})}}{\max_k(f_x)-\min_k(f_x)}.
\label{D_crowd}
\end{equation}

Based on Pareto set partition and crowding distance calculation, we sort the approximate circuits within each Pareto set in descending order of their $Dist$.
Subsequently, starting from the 0-ranked Pareto set, we sequentially select ${N}$ approximate circuits to form a new population for the next iteration.

After the non-dominated circuits sorting, the asymptotic error constraint relaxation is employed.
%to control the error constraint. 
We design a quadratic function scheme (i.e., $Error^{iter}_{cons.} = b\times iter^2 + Error^{0}_{cons.}$) to gradually increase the error constraint $Error^{iter}_{cons.}$ as the iteration $iter$ rises, ultimately relaxing it to the user-specified maximum error constraint by setting appropriate empirical parameter $b$.
% at the end of the optimization process.
This operation prevents the population from quickly moving to the maximum error constraint boundary and getting trapped in local optima.
%enables the population to search the solution space more comprehensively,


\subsection{Post-Optimization}
\label{GS}
%As mentioned in \Cref{sec:Intro}, we simultaneously target timing and area to overcome the issue of potential critical paths truncating the timing optimization. 
%Therefore, gate sizing is performed on the optimal approximate circuit generated by DCGWO, which can release the timing optimization potential embedded in the area, further decreasing the critical path delay.

%For approximate circuits with optimized critical path depth and area, enhancing the drive strength of gates can further release the timing optimization potential embedded in the area reduction.
%Therefore, post optimization is performed on the optimal approximate circuit generated by DCGWO.
Post-optimization is performed on the optimal approximate circuit generated by DCGWO.
It can further convert the area reductions into timing performance improvements by enhancing the drive strength of gates.

%During the previous process of approximate circuits generation, we did not remove the dangling gates (produced by the circuit searching and reproduction) from circuit netlist. 
We first delete dangling gates produced by circuit searching and reproduction from the optimal approximate circuit.
In this process, we traverse the entire circuit, identifying and removing gates with empty transitive fan-out (TFO).
For each fan-in of the removed gates, we similarly perform identification and removal operations until no gates with empty TFO remain.
Subsequently, for the processed optimal approximate circuit, we use Design Compiler \cite{designcompiler} to resize its remaining gates without adjusting any circuit structure under area constraints $\text{Area}_{con}$.
%By setting the timing constraint to 0, Design Compiler\cite{designcompiler} can enhance the drive strength of remaining gates as much as possible, minimizing critical path delay while increasing circuit area.
%To avoid excessive area growth, we manually set the area constraint to the original area of the corresponding accurate circuit.
%To fully convert area reduction into the enhancement of gate drive strength, we manually set the timing constraint to 0 and the area constraint $\text{Area}_{con}$ to the origin area of accurate circuit.
%In this case, Design Compiler\cite{designcompiler} can minimize critical path delay while increasing area to $\text{Area}_{con}$.  
Consequently, the final approximate circuits with minimum critical path delay $CPD_{fac}$ are obtained.




==> doc/abstract.tex <==
\begin{abstract}
With the shrinking technology nodes, timing optimization becomes increasingly challenging.
Approximate logic synthesis (ALS) can perform local approximate changes (LACs) on circuits to optimize timing with the cost of slight inaccuracy.
However, existing ALS methods that focus solely on critical path depth reduction (depth-driven methods) or area minimization (area-driven methods) are inefficient in achieving optimal timing improvement.
%Meanwhile, constructing effective ALS methods targeting both critical path depth and area remains tricky due to the dispersion of optimization gradients.
In this work, we propose an effective timing-driven ALS framework,
%based on double-chase grey wolf optimizer (DCGWO).
where we employ a double-chase grey wolf optimizer to explore and apply LACs, simultaneously bringing excellent critical path shortening and area reduction under error constraints.
%The framework employs DCGWO to simultaneously shorten critical path and reduce area under error constraints.
Subsequently, it utilizes post-optimization under area constraints to convert area reduction into further timing improvement, thus achieving maximum critical path delay reduction.
%Based on experiments using open-source circuits with TSMC 28nm technology, our framework can generate approximate circuits with optimal critical path delay reduction under different error and area constraints.
According to experiments on open-source circuits with TSMC 28nm technology, compared to the SOTA method, our framework can generate approximate circuits with greater critical path delay reduction under different error and area constraints.
%for random/control circuits, our framework achieves an average $27.13\%$ critical path delay reduction under a $5\%$ error rate constraint; for arithmetic circuits, our framework achieves an average $38.54\%$ critical path delay reduction under a $2.44\%$ normalized mean error distance constraint, both of which outperform the state-of-the-art.
\end{abstract}



==> doc/ack.tex <==
\iffalse
\section{Acknowledgment}
This work is supported by the National Natural Science Foundation of China under Grant 61874152 and 61904030 and The Research Grants Council of Hong Kong SAR (Project No.~CUHK24209017).
\fi

==> doc/conclu.tex <==
\section{Conclusion}
\label{sec:conclu}
In this work, we propose a timing-driven approximate logic synthesis framework based on DCGWO to effectively optimize circuit timing under $ER$ or $NMED$ constraints.
Its main idea involves using DCGWO to optimize both critical path depth and area to achieve precise and efficient optimal approximate circuit generation and utilizing post-optimization under area constraints to convert area reduction into further timing improvement.
According to the experimental results on open-source designs, under the same error and area constraints, our framework can achieve more critical path delay reduction than existing methods within an acceptable time consumption.
%Experimental results on open-source designs demonstrate that our framework can reduce critical path delay more efficiently than existing methods under the same error constraints.



\iffalse
In this work, we are the first to apply graph learning techniques to predict PBA timing results based on GBA results, addressing an important accuracy-runtime tradeoff in STA. 
Our work is composed of node embedding based on proposed EdgeGAT layers, predicting cell slew/delay synergistically based on node embedding results and calculating path arrival time through cumulative addition of predicted PBA cell delay values on timing path.
Compared with conventional graph learning methods, deep EdgeGAT can learn global path information. %, including cell features, net features and circuit structure, which helps improve predicting accuracy.
Experimental results on real-world open-source designs demonstrate that our predictor is both accurate and fast.
\fi


==> doc/experiment.tex <==

\section{Experimental Results}


Our proposed framework is implemented in Python.
We set up the experimental environment on the Linux machine with 32 cores and 4 NVIDIA Tesla V100 GPUs in parallel with 128GB memory. 
The benchmarks listed in \Cref{tab:benchmarks} are from ISCAS'85 \cite{hansen1999unveiling} and EPFL \cite{EPFL}. 
Each circuit is synthesized into gate-level netlist by Design Compiler \cite{designcompiler} under TSMC 28nm technology.
Among these benchmarks, random/control circuits are optimized under $ER$ constraints, while arithmetic circuits are optimized under $NMED$ constraints. 
For the generated approximate circuits, their timing-related information is obtained through static timing analysis performed by PrimeTime \cite{primetime}.
%The circuit error and similarities between gates outputs are derived through Monte Carlo-based logic simulation with a sample size of 20,000, executed by ABC.
The circuit error and the similarities between outputs of gates are obtained using VECBEE based on Monte Carlo simulation \cite{su2022vecbee}. 
By setting the number of sampled input vectors to $1\times 10^{5}$, this method can achieve fast error and similarities evaluation with nearly no deviation.

\subsection{Parameter Setting}
The parameters of our framework are set as follows.
%For population-related parameters, 
The population size ${N}$ is 30 and the upper limit of iterations $I_{max}$ is 20.
%In terms of circuit evaluation parameters, 
For PO-TFI pair evaluation function $Level$, $w_{\text{t}}$ is $0.9\times CPD_\text{ori}$ under both error constraints, while $w_{\text{e}}$ is respectively 0.1 and 0.2 under $ER$ and $NMED$ constraints.
For circuit fitness $Fit$, we determine the optimal weights based on \textbf{critical path delay ratios} of the final approximate circuits over the accurate circuits (i.e., $\text{Ratio}_{cpd}=\frac{CPD_{fac}}{CPD_\text{ori}}$). 
%traverse the value of $w_{\text{d}}$ in $\left [0,1 \right ] $ and
%the critical path depth weight $w_{\text{d}}$ and area weight $w_{\text{a}} = 1-w_{\text{d}}$ directly influence the optimization gradient.
%corresponding optimization results of the final approximate circuit, i.e., the critical path delay  ($CPD_{fac}$).
\Cref{weightchange} illustrates that the minimum $\text{Ratio}_{cpd}$ are achieved under both the tightest and loosest error constraints when $w_{\text{d}}$ is 0.8 and $w_{\text{a}} = 1-w_{\text{d}}$ is 0.2. 
Therefore, we follow this setting.
% For decision thresholds in double-chase, $S_{e}$ and $S_{\omega}$ equal 0.01 and 0.05 respectively.
% Reproduction rate $p_{re}$ is 0.6.
\begin{table}[t]
	\centering
	\caption{The benchmark statistics. $CPD_\text{ori}$ (ps) and $Area_\text{ori}$ ($\mu m^2$) respectively represents the \textbf{critical path delay} and area of accurate circuit.} 
\label{tab:benchmarks}
\resizebox{1.0\linewidth}{!}
{
    \Huge 
	\begin{tabular}{|c|lllcc|l|}
		\hline
		Type                       & Circuit    & \#gate & \#PI$/$PO & $CPD_\text{ori}$ & $Area_\text{ori}$  & Description              \\ \hline \hline
		  \multirow{2}{*}{}                   & Cavlc      & 573    & 10$/$11      & 186.35       & 450.31       & Coding Cavlc         \\
                                                & c880       & 322    & 60$/$26      & 185.34       & 177.67        & 8-bit ALU          \\
            Random$/$                           & c1908      & 366    & 33$/$25      & 235.14       & 223.34       & 16-bit SEC/DED circuit         \\
            Control                             & c2670      & 922    & 233$/$140     & 218.40      & 288.71       & 12-bit ALU and controller         \\
            \multirow{3}{*}{}                   & c3540      & 667    & 50$/$22      & 293.09       & 459.42       & 8-bit ALU         \\
                                                & c5315      & 2595   & 178$/$123     & 122.25      & 1129.55      & 9-bit ALU         \\
                                                & c7552      & 1576   & 207$/$108     & 282.13      & 939.33       & 32-bit adder/comparator         \\ \hline
                                                  
            \multirow{8}{*}{Arithmetic}         & Int2float  & 198    & 11$/$7      & 127.02        & 194.63       & int to float converter       \\ 
                                                & Adder16    & 269    & 32$/$17      & 58.92       & 288.41       & 16-bit adder          \\
                                                & Max16      & 154    & 32$/$16      & 131.78       & 91.43        & 16-bit 2-1 max unit          \\
                                                & c6288      & 1641   & 32$/$32      & 847.79       & 687.08       & 16$\times$16 multiplier         \\
                                                & Adder      & 1639   & 256$/$129     & 1394.7      & 495.78       & 128-bit adder            \\
		                                    & Max        & 2940   & 512$/$120    & 2799.8      & 954.03       & 128-bit 4-1 max unit     \\
		                                    & Sin        & 10962  & 24$/$25      & 701.03       & 4367.27      & 24-bit sine unit         \\ 
                                                & Sqrt       & 13542  & 128$/$64     & 67929.3       & 6262.10       & 128-bit square root unit    \\ \hline
            
		
	\end{tabular}
}
\vspace{-0.1in}
\end{table}

\begin{figure}[t!]
%\centering
\flushleft
\hspace{-.21in}
\subfloat[$ER$ Constraints]{\input{weightER} \label{fig:weightER}}
\hspace{-.23in}
\subfloat[$NMED$ Constraints]{\input{weightNMED} \label{fig:weightNMED}}	
\caption{Average critical path delay ratios $\text{Ratio}_{cpd}$ generated by our framework using different depth weight $w_{\text{d}}$ under the tightest and loosest $ER$ and $NMED$ constraints.}
%$w_{\text{cpd}}=0$ and $1$ respectively represents timing optimization targeting only area or timing.
\label{weightchange}
%\vspace{-0.05in}
\end{figure}


\begin{table*}[t!]
\centering
\caption{Comparison of performance between our framework and others under $5\%$ $ER$ constraints. All final generated circuits experience post-optimization under area constraints $\text{Area}_{con}$ to convert area reduction into further critical path delay reduction.}
\label{tab:er}
\resizebox{.94\linewidth}{!}
%\resizebox{8.8cm}{}}
{
\begin{tabular}{|l|c|cc|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{Circuit}   &{$\text{Area}_{con}$}  &\multicolumn{2}{c|}{VECBEE-S \cite{su2022vecbee}} &\multicolumn{2}{c|}{VaACS \cite{balaskas2022variability}}   &\multicolumn{2}{c|}{HEDALS\cite{meng2023hedals}}   &\multicolumn{2}{c|}{GWO (single-chase)}   &\multicolumn{2}{c|}{Ours} \\ 
                           &($\mu m^2$)          & $\text{Ratio}_{cpd}$         & runtime(s)        & $\text{Ratio}_{cpd}$          & runtime(s)     & $\text{Ratio}_{cpd}$          & runtime(s)      & $\text{Ratio}_{cpd}$     & runtime(s)   & $\text{Ratio}_{cpd}$          & runtime(s) \\ \hline \hline
Cavlc         &450.00  & 0.9219  & \textbf{60.03}  & 0.8745  & 356.89  &0.9071   &194.43   &0.8963   &407.25   & \textbf{0.8602}  & 310.42 \\
c880          &177.00  & 0.9026  & \textbf{43.11}  & 0.9221  & 227.13  &0.8913   &104.00   &0.9183   &201.51   & \textbf{0.8399}  & 193.86  \\
c1908         &223.00  & 0.8679  & \textbf{65.32}  & 0.5166  & 235.68  &\textbf{0.3372}   &310.42   &0.5021   &307.56   & 0.3865  & 202.79  \\
c2670         &288.00  & 0.6708 & 308.16 & 0.8101 & 477.92 &0.7589   &\textbf{250.28}   &0.7703   &313.99   & \textbf{0.6314} & 339.63 \\
c3540         &459.00  & 0.9670 & 391.42 & 0.9729 & 435.26 & 0.9203   &373.26   &0.9224   &479.88   & \textbf{0.8732} & \textbf{324.59} \\
c5315         &1129.00 & 0.9113 & 1857.32 & 0.8599 & 1963.55 &0.8270   &1662.08   &0.8165   &1655.07   & \textbf{0.8034} & \textbf{1449.37} \\
c7552         &939.00  & 0.9262 & 1726.27 & 0.9133  & 1336.64 &0.7391   &1315.85   &0.8877   &1420.32   & \textbf{0.7063}  & \textbf{1279.18} \\ \hline \hline 
Average       &523.57  & 0.8811 & 635.94 & 0.8385 & 719.01 &0.7687   &601.47   &0.8162   &683.65   & \textbf{0.7287} & \textbf{585.69} \\ \hline
\end{tabular}
}
\vspace{-0.01in}
\end{table*}

\begin{table*}[t!]
\centering
\caption{Comparison of performance between our framework and others under $2.44\%$ $NMED$ constraints. All final generated circuits experience post-optimization under $\text{Area}_{con}$ to convert area reduction into further critical path delay reduction.}
\label{tab:nmed}
\resizebox{.94\linewidth}{!}
%\resizebox{8.8cm}{}}
{ 
\begin{tabular}{|l|c|cc|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{Circuit}    &{$\text{Area}_{con}$}   & \multicolumn{2}{c|}{VECBEE-S \cite{su2022vecbee}} & \multicolumn{2}{c|}{VaACS \cite{balaskas2022variability}}    &\multicolumn{2}{c|}{HEDALS\cite{meng2023hedals}}   &\multicolumn{2}{c|}{GWO (single-chase)}   & \multicolumn{2}{c|}{Ours} \\ 
                                &($\mu m^2$)          & $\text{Ratio}_{cpd}$         & runtime(s)        & $\text{Ratio}_{cpd}$          & runtime(s)     & $\text{Ratio}_{cpd}$          & runtime(s)      & $\text{Ratio}_{cpd}$     & runtime(s)   & $\text{Ratio}_{cpd}$          & runtime(s) \\ \hline \hline
Int2float       &194.00  & 0.9331  & 71.23 & 0.5047  & 151.73 &0.7649 &\textbf{32.68} &0.6010 &178.30 & \textbf{0.4496}  & 132.12 \\
Adder16         &288.00  & 0.9973  & 67.20  & 0.5295  & 173.85  &0.4513 &\textbf{47.30} &0.5216 &189.01 & \textbf{0.4275}  & 167.03  \\
Max16           &91.00   & 0.7087  & \textbf{93.17} & 0.4209 & 189.73 &0.4470 &105.97 &0.3928 &277.38 & \textbf{0.3708} & 208.55 \\
c6288           &687.00  & 0.9663  & 4410.29  & 0.8696  & 3279.62  &\textbf{0.6368} &2563.41 &0.9079 &2991.00 & 0.8313  & \textbf{2103.88}  \\
Adder           &495.00  & 0.7814  & 1697.37  & 0.8133 & 2083.15  &0.7110 &1362.70 &0.8008 &1550.03 & \textbf{0.6917}  & \textbf{1193.71}  \\
Max             &954.00  & 0.8809  & 2600.78 & 0.8933 & 3397.50 &0.8355 &2992.08 &0.7517 &3121.44 & \textbf{0.6799} & \textbf{2035.62} \\
Sin             &4367.00 & 0.9187  & 5391.68  & 0.8326  & 3872.31  &0.7945 &3380.52 &0.8722 &4392.77 & \textbf{0.7603}  & \textbf{3176.46}  \\
Sqrt            &6262.00 & 0.7993  & 33117.12  & 0.8011  & 20160.76  &0.7437 &11242.29 &0.7803 &17894.50 & \textbf{0.7058}  & \textbf{9950.11}  \\ \hline \hline
Average         &1667.25 & 0.8732   & 5931.11  & 0.7081  & 4163.58 &0.6731 &2715.87 &0.7035 &3824.30 & \textbf{0.6146} & \textbf{2370.94} \\ \hline
\end{tabular}
}
\vspace{-0.16in}
\end{table*}

\subsection{Optimization Performance}
Since our framework focuses on timing optimization, we compare the performance of our framework, including final \textbf{critical path delay ratios} $\text{Ratio}_{cpd}=\frac{CPD_{fac}}{CPD_\text{ori}}$ and \textbf{runtime}, with: (1) area-driven methods: VECBEE-SASIMI \cite{su2022vecbee}; (2) depth-driven methods: VaACS \cite{balaskas2022variability}, HEDALS \cite{meng2023hedals}; (3) traditional GWO (single-chase). 
%(1) VECBEE-SASIMI \cite{su2022vecbee} focusing on area minimization and (2) VaACS \cite{balaskas2022variability} focusing on critical path depth reduction.
% Both (1) and (2) are modified to adapt to our timing optimization scenario, 
Approximate circuits generated by these works experience post-optimization (in \Cref{GS}) under \textbf{area constraints} $\text{Area}_{con}$ to convert area reduction into further critical path delay reduction by Design Compiler {\cite{designcompiler}}. 

%For random/control circuits, the performance comparison of all works under the loosest $5\%$ $ER$ constraint is detailed in \Cref{tab:er}. 


%For random/control circuits, \Cref{fig:ERcon} shows the average $\text{Ratio}_{cpd}$ of three excellent works under 5 different $ER$ constraints ($1\%$, $2\%$, $3\%$, $4\%$ and $5\%$), while the performance comparison of all works under the loosest $5\%$ $ER$ constraint is detailed in \Cref{tab:er}. 
%According to the comparison results, by setting the same area constraints, our framework maximizes the average critical path delay reduction to $27.13\%$ with shorter runtime under $5\%$ $ER$ constraint.
%Meanwhile, as the $ER$ constraint tightens, our framework consistently achieve greater critical path delay reductions.
%the timing results of our framework and others under $ER$ constraints of $1\%$, $2\%$, $3\%$, $4\%$ and $5\%$ is shown in \Cref{fig:ERcon}.
%It indicates that our framework can reduce more critical path delay under all $ER$ constraints.
% achieving better approximate timing optimization.
%\Cref{tab:er} summarizes the performance of all works under the loosest $ER$ constraint of $5\%$. 
%reflecting the optimal performance of approximate timing optimization.
%According to the result, our framework can maximize the average critical path delay reduction to $27.13\%$, further optimizing by $15.24\%$ and $10.98\%$ compared to VECBEE-SASIMI \cite{su2022vecbee} and the NSGA-II-based approach \cite{balaskas2022variability}, respectively.

%For arithmetic circuits, the timing results of our framework and others under $NMED$ constraints of $0.48\%$, $0.98\%$, $1.47\%$, $1.96\%$ and $2.44\%$ is illustrated in \Cref{fig:NMEDcon}.
%It indicates that our framework can achieve superior timing optimization under all $NMED$ constraints.
%As shown in \Cref{tab:nmed}, our framework can maximize the average critical path delay reduction to $38.54\%$ under the loosest $NMED$ constraint of $2.44\%$, further optimizing by $25.86\%$ and $9.35\%$ compared to VECBEE-SASIMI \cite{su2022vecbee} and the NSGA-II-based approach \cite{balaskas2022variability}, respectively.

For random/control circuits, the performance comparison of all works under the loosest $5\%$ $ER$ constraint is detailed in \Cref{tab:er}. 
According to the comparison results, by setting the same area constraints, our framework maximizes the average critical path delay reduction to $27.13\%$ with shorter runtime under the $5\%$ $ER$ constraint.
Similarly, for arithmetic circuits, the performance comparison of all works under the loosest $2.44\%$ $NMED$ constraint is detailed in \Cref{tab:nmed}.
The comparison results indicate that our framework maximizes the average critical path delay reduction to $38.54\%$ with shorter runtime under the $2.44\%$ $NMED$ constraint.

\begin{figure}[t!]
%\centering
\flushleft
\hspace{-.2in}
\subfloat[Random/Control Circuits]{\input{ERcon} \label{fig:ERcon}}
\hspace{-.23in}
\subfloat[Arithmetic Circuits]{\input{NMEDcon} \label{fig:NMEDcon}}	
\caption{Average critical path delay ratios $\text{Ratio}_{cpd}$ generated by our framework, HEDALS \cite{meng2023hedals} and traditional GWO under different $ER$ and $NMED$ constraints.}
\label{underconstraint}
\vspace{-0.02in}
\end{figure}

% Similarly, for arithmetic circuits, \Cref{fig:NMEDcon} shows the average $\text{Ratio}_{cpd}$ of three excellent works under 5 different $NMED$ constraints ($0.48\%$, $0.98\%$, $1.47\%$, $1.96\%$ and $2.44\%$), while the performance comparison of all works under the loosest $2.44\%$ $NMED$ constraint is detailed in \Cref{tab:nmed}.
%According to the comparison results, our framework maximizes the average critical path delay reduction to $38.54\%$ with shorter runtime under the $2.44\%$ $NMED$ constraint.
%while achieving an average $2.5\times$ and $1.76\times$ runtime speedup compared to \cite{su2022vecbee} and \cite{balaskas2022variability}.
%Meanwhile, as the $NMED$ constraint tightens, our framework continues to achieve greater critical path delay reductions.

We further compare the average $\text{Ratio}_{cpd}$ achieved by our work with HEDALS\cite{meng2023hedals} and traditional GWO under 5 different $ER$ constraints ($1\%$, $2\%$, $3\%$, $4\%$, $5\%$)  and 5 different $NMED$ constraints ($0.48\%$, $0.98\%$, $1.47\%$, $1.96\%$, $2.44\%$). 
According to results in \Cref{underconstraint}, as the $ER$ or $NMED$ constraint tightens, our framework consistently achieves greater critical path delay reductions than others.
\Cref{underAreaconstraint} illustrates how the average $\text{Ratio}_{cpd}$ varies with different area constraints ($0.8\times \sim1.2 \times$ $\text{Area}_{con}$) under the loosest $ER$ and $NMED$ constraints.  
The results indicate that our framework outperforms other works in timing optimization across all area constraints.
These achievements demonstrate that our framework can generate approximate circuits with superior performance while meeting diverse accuracy and area requirements.


\begin{figure}[t!]
%\centering
\flushleft
\hspace{-.2in}
\subfloat[$5\%$ $ER$ Constraint]{\input{AreaconER} \label{fig:AreaconER}}
\hspace{-.23in}
\subfloat[$2.44\%$ $NMED$ Constraint]{\input{AreaconNMED} \label{fig:AreaconNMED}}	
\caption{Average critical path delay ratios $\text{Ratio}_{cpd}$ generated by our framework, HEDALS \cite{meng2023hedals} and traditional GWO under different area constraints ($\text{Ratio} \times \text{Area}_{con}$).}
\label{underAreaconstraint}
\vspace{-0.015in}
\end{figure}

In summary, by leveraging carefully designed approximate actions and the powerful search capabilities of DCGWO, our framework can better exploit the timing improvement inherent in critical path shortening and the enhancement of gate drive strength.
Additionally, compared to traditional GWO, using the double-chase strategy to further formulate the optimization gradients indeed helps the optimizer find better solutions.
Benefiting from the fast implementation of LACs and the inherent parallelism of GWO, our framework maintains low time consumption despite using PrimeTime \cite{primetime} for accurate timing analysis.






\iffalse
\begin{table}[t!]
\centering
\caption{Comparison of performance between our framework and others \cite{su2022vecbee,balaskas2022variability,meng2023hedals} under $5\%$ $ER$ constraints.}
\label{tab:er}
\resizebox{1.0\linewidth}{!}
%\resizebox{8.8cm}{}}
{ 
\Large
\begin{tabular}{|l|c|cc|cc|cc|}
\hline
\multirow{2}{*}{Circuit}   &\multirow{2}{*}{$\text{Area}_{con}$}  & \multicolumn{2}{c|}{VECBEE-S \cite{su2022vecbee}} & \multicolumn{2}{c|}{VaACS \cite{balaskas2022variability}} & \multicolumn{2}{c|}{Ours} \\ 
                           &          & $\text{Ratio}_{cpd}$         & $rt$(s)        & $\text{Ratio}_{cpd}$          & $rt$(s)       & $\text{Ratio}_{cpd}$          & $rt$(s)    \\ \hline \hline
Cavlc         &450.00  & 0.9219  & \textbf{60.03}  & 0.8745  & 356.89  & \textbf{0.8602}  & 310.42 \\
c880          &177.00  & 0.9026  & \textbf{43.11}  & 0.9221  & 227.13  & \textbf{0.8399}  & 193.86  \\
c1908         &223.00  & 0.8679  & \textbf{65.32}  & 0.5166  & 235.68  & \textbf{0.3865}  & 202.79  \\
c2670         &288.00  & 0.6708 & \textbf{308.16} & 0.8101 & 477.92 & \textbf{0.6314} & 339.63 \\
c3540         &459.00  & 0.9670 & 391.42 & 0.9729 & 435.26 & \textbf{0.8732} & \textbf{324.59} \\
c5315         &1129.00 & 0.9113 & 1857.32 & 0.8599 & 1963.55 & \textbf{0.8034} & \textbf{1449.37} \\
c7552         &939.00  & 0.9262 & 1726.27 & 0.9133  & 1336.64 & \textbf{0.7063}  & \textbf{1279.18} \\ \hline \hline 
Average       &523.57  & 0.8811 & 635.94 & 0.8385 & 719.01 & \textbf{0.7287} & \textbf{585.69} \\ \hline
\end{tabular}
}
\vspace{-0.1in}
\end{table}


\begin{table}[t!]
\centering
\caption{Comparison of performance between our framework and others \cite{su2022vecbee}, \cite{balaskas2022variability} under $2.44\%$ $NMED$ constraints.}
\label{tab:nmed}
\resizebox{1.0\linewidth}{!}
%\resizebox{8.8cm}{}}
{ 
\Large
\begin{tabular}{|l|c|cc|cc|cc|}
\hline
\multirow{2}{*}{Circuit}    &\multirow{2}{*}{$\text{Area}_{con}$}   & \multicolumn{2}{c|}{VECBEE-S \cite{su2022vecbee}} & \multicolumn{2}{c|}{CaACS \cite{balaskas2022variability}} & \multicolumn{2}{c|}{Ours} \\ 
                                &           & $\text{Ratio}_{cpd}$        & $rt$(s)        & $\text{Ratio}_{cpd}$          & $rt$(s)       & $\text{Ratio}_{cpd}$          & $rt$(s)    \\ \hline \hline
Int2float       &194.00  & 0.9331  & \textbf{71.23} & 0.5047  & 151.73 & \textbf{0.4496}  & 132.12 \\
Adder16         &288.00  & 0.9973  & \textbf{67.20}  & 0.5295  & 173.85  & \textbf{0.4275}  & 167.03  \\
Max16           &91.00   & 0.7087  & \textbf{93.17} & 0.4209 & 189.73 & \textbf{0.3708} & 208.55 \\
c6288           &687.00  & 0.9663  & 4410.29  & 0.8696  & 3279.62  & \textbf{0.8313}  & \textbf{2103.88}  \\
Adder           &495.00  & 0.7814  & 1697.37  & 0.8133 & 2083.15  & \textbf{0.6917}  & \textbf{1193.77}  \\
Max             &954.00  & 0.8809  & 2600.78 & 0.8933 & 3397.50 & \textbf{0.6799} & \textbf{2035.62} \\
Sin             &4367.00 & 0.9187  & 5391.68  & 0.8326  & 3872.31  & \textbf{0.7603}  & \textbf{3176.46}  \\
Sqrt            &6262.00 & 0.7993  & 33117.12  & 0.8011  & 20160.76  & \textbf{0.7058}  & \textbf{9950.11}  \\ \hline \hline
Average         &1667.25 & 0.8732   & 5931.11  & 0.7081  & 4163.58 & \textbf{0.6146} & \textbf{2370.94} \\ \hline
\end{tabular}
}
\vspace{-0.09in}
\end{table}


\Cref{opt} demonstrates the comparison of average optimization runtime across different works. 
Since our framework performs optimization based on accurate timing information, it is more time-consuming than VECBEE-SASIMI \cite{su2022vecbee}. 
Compared to the NSGA-II-based approach \cite{balaskas2022variability}, our framework converges to optimal solutions in fewer iterations due to the consideration of gradients, resulting in shorter runtime.
According to the optimization results and runtime, our framework is more efficient than VECBEE-SASIMI \cite{su2022vecbee} and the NSGA-II-based approach \cite{balaskas2022variability} in approximate timing optimization.
%the runtime of our framework is slower than VECBEE-SASIMI \cite{su2022vecbee}, and slightly faster than the NSGA-II-based approach \cite{balaskas2022variability}. The reason behind this is that our framework does not terminate prematurely due to being trapped in local optima like VECBEE-SASIMI \cite{su2022vecbee}, and can converge to the optimal solutions in fewer iterations than the NSGA-II-based approach \cite{balaskas2022variability}.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{opt.pdf}
    \caption{Average optimization runtime ($min.$) of our framework and others under $5\%$ $ER$ and $2.44\%$ $NMED$ constraints.}
    \label{opt}
\end{figure}




\begin{table}[t]
\centering
\caption{Performance comparison of our framework with others \cite{su2022vecbee}, \cite{balaskas2022variability} under $5\%$ $ER$ constraints.}
\label{tab:er}
\resizebox{1.0\linewidth}{!}
%\resizebox{8.8cm}{}}
{ 
\LARGE
\begin{tabular}{|l|cc|cc|cc|}
\hline
\multirow{2}{*}{Circuit}   & \multicolumn{2}{c|}{VECBEE-SASIMI \cite{su2022vecbee}} & \multicolumn{2}{c|}{NSGA-II \cite{balaskas2022variability}} & \multicolumn{2}{c|}{Ours} \\ 
                                     & $\text{Ratio}_{cpd}$         & runtime(s)        & $\text{Ratio}_{cpd}$          & runtime(s)       & $\text{Ratio}_{cpd}$          & runtime(s)    \\ \hline \hline
c880          & 0.9026  & \textbf{43.11}  & 0.9221  & 127.13  & \textbf{0.8399}  & 93.86  \\
c1908         & 0.8679  & \textbf{65.32}  & 0.5845  & 135.68  & \textbf{0.3865}  & 102.79  \\
c2670         & 0.7408 & 143.53 & 0.8101 & 177.92 & \textbf{0.6314} & \textbf{139.63} \\
c3540         & 0.9670 & 137.96 & 0.9729 & 163.26 & \textbf{0.8732} & \textbf{124.34} \\
c7552         & 0.9262 & 332.17 & 0.9133  & 336.64 & \textbf{0.8063}  & \textbf{279.18} \\
cavlc         & 0.9219  & \textbf{60.03}  & 0.8745  & 156.89  & \textbf{0.8602}  & 110.42  \\ \hline \hline
Average       & 0.8877 & \textbf{130.36} & 0.8462 & 182.92 & \textbf{0.7329} & 141.70 \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[t]
\centering
\caption{Performance comparison of our framework with others \cite{su2022vecbee}, \cite{balaskas2022variability} under $2.44\%$ $NMED$ constraints.}
\label{tab:nmed}
\resizebox{1.0\linewidth}{!}
%\resizebox{8.8cm}{}}
{ 
\LARGE
\begin{tabular}{|l|cc|cc|cc|}
\hline
\multirow{2}{*}{Circuit}   & \multicolumn{2}{c|}{VECBEE-SASIMI \cite{su2022vecbee}} & \multicolumn{2}{c|}{NSGA-II \cite{balaskas2022variability}} & \multicolumn{2}{c|}{Ours} \\ 
                                           & $\text{Ratio}_{cpd}$        & runtime(s)        & $\text{Ratio}_{cpd}$          & runtime(s)       & $\text{Ratio}_{cpd}$          & runtime(s)    \\ \hline \hline
Adder16         & 0.9973  & \textbf{31.20}  & 0.5295  & 73.85  & \textbf{0.4275}  & 67.03  \\
Adder           & 0.7814  & 1697.37  & 0.8133 & 1083.15  & \textbf{0.6917}  & \textbf{593.77}  \\
Max16           & 0.7087  & \textbf{46.17} & 0.4209 & 89.73 & \textbf{0.3708} & 76.55 \\
Max             & 0.8809  & 2600.78 & 0.8933 & 2397.50 & \textbf{0.6799} & \textbf{1035.62} \\
Int2float       & 0.9331  & \textbf{11.23} & 0.5047  & 71.73 & \textbf{0.4496}  & 62.12 \\
c6288           & 0.9663  & 3410.29  & 0.8696  & 1279.62  & \textbf{0.8313}  & \textbf{1103.88}  \\
Sin             & 0.9187  & 3391.68  & 0.8326  & 2872.31  & \textbf{0.7603}  & \textbf{2176.46}  \\
Sqrt            & 0.7993  & 43117.12  & 0.8011  & 30160.76  & \textbf{0.7058}  & \textbf{9950.11}  \\ \hline \hline
Average        & 0.8732   & 6788.23  & 0.7081  & 4753.58 & \textbf{0.6146} & \textbf{1883.19} \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[t!]
\centering
\caption{Comparison of performance between our framework and others \cite{su2022vecbee}, \cite{balaskas2022variability} under $5\%$ $ER$ constraints.}
\label{tab:er}
\resizebox{1.0\linewidth}{!}
%\resizebox{8.8cm}{}}
{ 
\LARGE
\begin{tabular}{|l|cc|cc|cc|}
\hline
\multirow{2}{*}{Circuit}   & \multicolumn{2}{c|}{VECBEE-SASIMI \cite{su2022vecbee}} & \multicolumn{2}{c|}{NSGA-II \cite{balaskas2022variability}} & \multicolumn{2}{c|}{Ours} \\ 
                                     & $\text{Ratio}_{cpd}$         & runtime(s)        & $\text{Ratio}_{cpd}$          & runtime(s)       & $\text{Ratio}_{cpd}$          & runtime(s)    \\ \hline \hline
Cavlc         & 0.9219  & \textbf{60.03}  & 0.8745  & 356.89  & \textbf{0.8602}  & 310.42 \\
c880          & 0.9026  & \textbf{43.11}  & 0.9221  & 227.13  & \textbf{0.8399}  & 193.86  \\
c1908         & 0.8679  & \textbf{65.32}  & 0.5845  & 235.68  & \textbf{0.3865}  & 202.79  \\
c2670         & 0.7408 & \textbf{308.16} & 0.8101 & 477.92 & \textbf{0.6314} & 339.63 \\
c3540         & 0.9670 & 391.42 & 0.9729 & 435.26 & \textbf{0.8732} & \textbf{324.59} \\
c5315         & 0.9670 & 1857.32 & 0.9729 & 1963.55 & \textbf{0.8732} & \textbf{1449.37} \\
c7552         & 0.9262 & 1726.27 & 0.9133  & 1336.64 & \textbf{0.8063}  & \textbf{1279.18} \\ \hline \hline 
Average       & 0.8877 & 635.94 & 0.8462 & 719.01 & \textbf{0.7329} & \textbf{585.69} \\ \hline
\end{tabular}
}
\vspace{-0.1in}
\end{table}
\fi

==> doc/intro.tex <==
\section{Introduction}
\label{sec:Intro}
Timing optimization is crucial in VLSI design.
As the CMOS technology nodes continue to shrink, timing improvements caused by traditional methods, including gate sizing and logic restructure, are 
limited \cite{esmaeilzadeh2011dark, han2013approximate}.
In recent years, error-tolerant applications are becoming increasingly popular.
%In recent years, circuit functions have increasingly focused on error-tolerant applications such as video processing and machine learning.
Consequently, approximate computing \cite{han2013approximate}, which effectively balances accuracy and performance, has garnered great attention.
%from designers.
It can significantly reduce circuit delay, area, and power with the cost of slight computational imprecision.
%By substituting the original circuit for an approximate version with slight computational imprecision, it can significantly reduce circuit delay, area, and power \cite{su2022vecbee}.

\iffalse
Recently, some studies have proposed an automated approximate computing paradigm, i.e., approximate logic synthesis (ALS) \cite{su2022vecbee,lee2023approximate,balaskas2021automated,balaskas2022variability,ye2024timing,hashemi2018blasys,meng2022seals}.
It can optimize timing by reducing the depth of critical paths and enhancing the drive strength of gates on critical paths \cite{ye2024timing}.
 \Cref{gca} gives examples of local approximate changes (LACs) used in ALS to generate approximate solutions for timing optimization.
Since LACs are fast and easy to achieve on circuits, they are always combined with complex heuristic algorithms
\cite{su2022vecbee,lee2023approximate,balaskas2021automated,balaskas2022variability,ye2024timing,hashemi2018blasys}.
As shown in \Cref{gradient}, these combinatorial optimization methods often focus on two categories: (1) directly optimizing area, which can be converted into the enhancement of gates drive strength for timing improvement.
VECBEE-SASIMI \cite{su2022vecbee} combines efficient error evaluation with a greedy algorithm to conduct fast approximate area optimization.
(2) directly optimizing critical path depth, which can bring immediate timing improvement.
VaACS \cite{balaskas2022variability} use a non-dominated sorting genetic algorithm (NSGA-II) to perform variability-Aware approximation on critical paths. 
%(2) directly optimizing critical path depth.
%NSGA-II-based approach \cite{balaskas2022variability} and TTMA-RL \cite{ye2024timing} respectively use a non-dominated sorting genetic algorithm (NSGA-II) and reinforcement learning method for LACs selection to reduce critical path depth directly.
%ALS-ERG \cite{lee2023approximate} performs circuit partition and approximation based on a genetic algorithm, aiming to reduce circuit depth.
\fi

Recently, approximate logic synthesis (ALS) has been proposed as an automated approximate computing paradigm.
It can optimize timing under a relaxed error bound by reducing the depth of critical paths and enhancing the drive strength of gates on critical paths \cite{ye2024timing}.
%Existing ALS methods mainly focus on two categories: (1) decreasing critical path depth (i.e., depth-only) \cite{balaskas2021automated,balaskas2022variability,lee2023approximate} or (2) reducing area (i.e., area-only) \cite{su2022vecbee,meng2022seals,meng2020alsrac}.
Based on optimization approaches, existing ALS methods can primarily be divided into two categories: (1) depth-driven methods \cite{balaskas2021automated,balaskas2022variability,meng2023hedals} and (2) area-driven methods \cite{meng2020alsrac,meng2022seals,su2022vecbee,lee2023approximate}.
Depth-driven methods perform local approximate changes (LACs) to simplify gates on critical paths, providing direct timing improvement.
As shown in \Cref{gca}, LACs are applied to critical paths 1 and 2.
By omitting certain gates, both paths become shallower and faster with the cost of a slight error.
HEDALS \cite{meng2023hedals} proposes a critical error graph to accelerate critical path depth reduction and strictly control the introduced errors.
%HEDALS \cite{meng2023hedals} proposes a critical error graph to accelerate the aforementioned process and strictly control the introduced errors.
%which decreases the depth of critical paths and provides direct timing improvement.
Area-driven methods select LACs with the best area reduction potential to minimize circuit area. 
SEALS \cite{meng2022seals} and VECBEE-SASIMI \cite{su2022vecbee} combine fast error estimation with greedy algorithms to iteratively select such LACs, efficiently reducing circuit area.
\Cref{gca} also illustrates that these area reductions can be converted into the enhancement of gate drive strength by post-optimization, leading to further timing improvement.
%Since area reduction can be converted into the enhancement of gate drive strength.

However, achieving ALS with the greatest potential for timing optimization is challenging for previous methods. 
%that directly optimize critical path depth or area. 
%use the number of gates on the deepest path as a substitute for accurate delay information.
%during the optimization process.
Specifically, depth-driven methods inadequately reduce area, leading to difficulties in maximizing the drive strength of gates on critical paths.
%for depth-driven methods, numerous potential critical paths in the later stages of optimization lead to the gradient vanishing of further timing improvement.
Area-driven methods simplify many gates on non-critical paths to reduce area, which makes it difficult to obtain the optimal critical path depth.
%It causes the optimization to terminate prematurely.
%For methods targeting only timing \cite{balaskas2021automated}\cite{ye2024timing}, there is a risk of too many potential critical paths emerging in the later stages of optimization, making the gradient of timing optimization disappear, and prematurely terminating the optimization process \cite{hashemi2018blasys}.
%Therefore, it is necessary to target both timing and area during timing optimization. 
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\linewidth]{LACs.pdf}
    \caption{Optimizing circuit by wire-by-wire (substitute a wire with another wire in circuits) and wire-by-constant (substitute a wire with constant logic value `0'$/$`1') LACs. Area reductions are converted into drive strength enhancement of gates.}
    \label{gca}
\vspace{-0.03in}
\end{figure}
% gradient
%\begin{figure}
%    \centering
%    \includegraphics[width=1\linewidth]{Pareto2.pdf}
%    \caption{Approximate optimization results (before gate sizing) using different methods under the same error constraint.}
%    \label{gradient}
%\vspace{-0.2in}
%\end{figure}
% figure end
Therefore, it is necessary for timing-driven ALS to simultaneously optimize both critical path depth and area. 
In this scenario, conventional gradient-based optimizers, including greedy algorithm, genetic algorithm, and traditional grey wolf optimizer (GWO) \cite{mirjalili2016multi} using a single-chase strategy, cannot finely partition the sampled approximate solutions.
Thus, solutions are dispersed in the solution space.
% As shown in lower part of \Cref{gradient}.
This dispersion causes an excessive number of gradients for further optimization.
It makes solutions easily move along the gradient with the current fastest critical path depth shortening or area reduction.
Finally, traditional optimizers fall into local optima \cite{zheng2023mitigating, zhao2021multi}.
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=.98\linewidth]{overallflow1.pdf}
    \caption{The overall flow of our timing-driven approximate logic synthesis framework based on double-chase grey wolf optimizer.}
    \label{Overflow}
\vspace{-0.1in}
\end{figure*}

In this work, we propose a timing-driven approximate logic synthesis framework. 
As shown in \Cref{Overflow}, the framework is composed of three steps, including circuit representation, the double-chase grey wolf optimizer (DCGWO), and post-optimization.
Firstly, adjacency lists are constructed based solely on gate fan-in relationships to enable fast circuit structure storage and LACs application.
Then, DCGWO efficiently optimizes both critical path depth and area under error constraints.
Subsequently, post-optimization under area constraints converts the area reduction into further timing optimization.
%The framework automatically optimizes both critical path delay and area under error constraints of error rate or normalized mean error distance, and convert area reduction into timing optimization for maximum critical path delay reduction through gate sizing under area constraints.
%Our DCGWO precisely partitions the generated approximate circuits into finer hierarchies and formulates appropriate approximate optimization gradients for each hierarchy, accelerating the efficiency in finding the global optimal approximate circuit.
Our contributions are summarized as follows:

\begin{itemize}
\item We propose a framework for deeply exploiting timing improvement inherent in the reduction of critical path depth and the enhancement of gate drive strength.
%multi-objective timing optimization targeting both circuit depth and area to minimize critical path delay under error constraints.
\item We represent accurate and approximate circuits based on gate fan-in adjacency lists to improve storage efficiency and accelerate timing optimization.
\item We present a DCGWO to effectively select approximate actions for reducing critical path depth and area.
Building upon traditional GWO, it divides the generated approximate circuit population into finer hierarchies and precisely formulates appropriate optimization gradients for each hierarchy, improving the efficiency in finding the global optimal approximate circuit.
%by partitioning the iteratively generated approximate circuits into different hierarchies and designing specific approximate actions for them.
\item The experimental results demonstrate that our framework achieves an average $27.13\%$ and $38.54\%$ critical path delay reduction respectively, under a $5\%$ error rate constraint and under a $2.44\%$ normalized mean error distance constraint, outperforming the state-of-the-art method.
\end{itemize}



==> doc/key.tex <==
\begin{keywords}
Timing Optimization, Approximate Logic Synthesis, Double-chase Grey Wolf Optimizer, Gate Sizing
\end{keywords}


==> doc/preliminaries.tex <==
\section{Preliminaries}
\iffalse
\subsection{Gate-level Circuit Approximation}
\label{sec:model}
The LACs used in our framework includes wire-by-wire \cite{venkataramani2013substitute} and wire-by-constant \cite{schlachter2017design} replacements applied to the gate-level netlist. 
%These state-of-the-art LACs are highly process-dependent and easy to implement, allowing for a good consideration of the circuit actual timing, area and error.
Wire-by-wire replacement refers to substituting a wire (target wire) in the circuit with another one (switch wire).
An example of wire-by-wire replacement is illustrated in \Cref{gca}, where target wire $w{\text{7}}$ is substituted by switch wire $w{\text{3}}$.
This substitution decreases the depth of $path1$ with the cost of $12.5\%$ error rate, accelerating $path1$ and reducing circuit area by neglecting gates $U{\text{2}}$ and $U{\text{4}}$.
% wire-by-wire and wire-by-constant
%figure end
Wire-by-constant replacement refers to replacing the target wire with the constant logic value `0' or `1'.
As shown in \Cref{gca}, target wire $w{\text{14}}$ is replaced by the constant logic value `1'.
Thus, $path2$ becomes shallower and faster by omitting gates $U{\text{3}}$ and $U{\text{6}}$ with almost no error cost.
\fi
\iffalse
In summary, these two LACs can potentially reduce the critical path delay of circuits.
However, they will inevitably introduce logic errors.
Furthermore, as circuits become larger, the solution space expands significantly, making it challenging to find optimal solutions.
To limit errors and the solution space, a common approach is to select LACs based on logic similarity \cite{balaskas2021automated} \cite{hashemi2018blasys}.  
For target wire $n_{i}$, we obtain the percentage of cycles when $n_{i}$ holds the same value with constant `0', constant `1' and all switch wire candidates, which are expressed as similarities $S_{n_{i}}^{\text {0}}$, $S_{n_{i}}^{\text {1}}$ and $\{S_{n_{i}}^{n_{a}}, ..., S_{n_{i}}^{n_{b}}\} $. 
The constant or wire candidate corresponding to the similarity $ max \{S_{n_{i}}^{\text {0}}, S_{n_{i}}^{\text {1}}, S_{n_{i}}^{n_{a}}, ... , S_{n_{i}}^{n_{b}}\}$ will be selected.
\fi

\subsection{Error Metrics}
\label{sec:metrics}
The error metrics used in our framework are error rate ($ER$) and normalized mean error distance ($NMED$). $ER$ can be used to measure the error of random/control circuits, while $NMED$ can evaluate the error of arithmetic circuits. 

For a circuit with $m$ primary inputs and $n$ primary outputs, we assume the probability of input vector $I_{i}$ occurring is $p_{i}$, where $1 \leq i \leq  2^m$. 
In this case, $ER$ is the probability that the approximate circuit output differs from the accurate circuit output, calculated by \Cref{eq:ER}, where $O_{i}^{\text {app}}$ and $O_{i}^{\text {ori}}$ are output vectors of the approximate circuit and accurate circuit for input vector $I_{i}$.
\begin{equation}
ER = \sum \limits_{i=1}^{2^m} (O_{i}^{\text {app}}\ne O_{i}^{\text {ori}})\times p_{i}.
\label{eq:ER}
\end{equation}

Error distance is the difference between approximate circuit output value $V_{i}^{\text {app}}$ and accurate circuit output value $V_{i}^{\text {ori}}$ under input vector $I_{i}$.
$NMED$ is the mean error distance normalized by the maximum output value, defined in \Cref{eq:NMED}. 
\begin{equation}
NMED = \sum \limits_{i=1}^{2^m}
\frac{\left | V_{i}^{\text {ori}} - V_{i}^{\text {app}} \right |}{2^n - 1}\times p_{i}.
\label{eq:NMED}
\end{equation}

%To reduce the scale of error analysis and further enhance the efficiency of evaluation process, we employed a method based on Monte Carlo simulation, derived from VECBEE \cite{su2022vecbee}.
%Compared to the traditional full-input pattern traversal method, by setting the number of sample points to over 10,000, this Monte Carlo-based method can achieve faster error evaluation with nearly no deviation.

\subsection{Problem Formulation}
\label{ProF}
As introduced in \Cref{sec:Intro}, optimizing both critical path depth and area can effectively exploit the potential timing improvement inherent in critical path depth reduction and the enhancement of gate drive strength.
Thus, the timing-driven ALS problem can be formulated as follows:
% as a multi-objective optimization considering both timing and area under error constraints as follows:
\begin{myproblem}[Timing-driven ALS]
\label{pro:1}
\textit{Given a post-synthesis netlist of the accurate circuit with timing, area, and logic information, use an approximate optimizer simultaneously optimizing both critical path depth and area under error constraints to generate the final approximate circuit with maximum critical path delay reduction.}
\end{myproblem}


\iffalse
\subsection{Motivation}
\label{sec:DCGWO}
As introduced in \cref{sec:Intro}, the optimal combination algorithm generated by combining ALS with heuristic algorithms can better optimize circuits.
For large circuits, the solution space for approximate actions is vast.
Gradient-based optimizer, including genetic algorithms and traditional grey wolf optimizer (GWO) could not finely partition the sampled solutions, resulting in solutions being dispersed in the solution space.
This dispersion leads to an excessive number of gradients for further optimization, making solutions easily move in the direction of the steepest fitness gradient, and thus fall into local optima.


To solve this problem, as shown in \Cref{patition}, we partition the approximate solutions generated in each iteration into optimal solution, sub-optimal solutions and remaining solutions based on their performance in terms of delay and area. 
Furthermore, we capture the performance gap between solutions at different hierarchies to set specific approximate actions.
This approach enhances the diversity of approximate solutions and increases the specificity of the search, accelerating the efficiency in finding the optimal solution.

\subsection{Why Double-chase Grey Wolf Optimizer?}
\label{sec:DCGWO}
Grey wolf optimizer (GWO) is a swarm intelligence algorithm inspired by wolves hunting.
It classifies the population based on fitness, and performs further chasing within each classification to find the optimal solution in the solution space.
When GWO is applied to approximate optimization, it selects approximate circuits with better delay, area based on fitness evaluation and uses them to guide the generation of new approximate circuits, making the search for the optimal approximate solution more purposeful and efficient than genetic algorithm and greed optimization.

In the traditional GWO, there is only a single-chase mechanism where individuals update their information by chasing the leader wolves (the top three individuals in terms of fitness).
For large circuits, the increase in wires and paths leads to a vast number of potential approximate operations, significantly expanding the solution space for optimization.
In this scenario, the single-chase GWO lacks sufficient search capability, making the search for the optimal approximate solution slow and prone to getting stuck in local optima.

To address this, we employed a double-chase strategy to improve GWO. 
As shown in Fig. 2, the population is divided into three classes.
Specifically, the leader is defined as the approximate circuit with the highest fitness in the circuit population, guiding three elite circuits with fitness ranks 2, 3, and 4 to conduct the chase.
The elite circuits, in turn, guide the remaining circuits in their chase.
By formulating appropriate search and convergence schemes for these two chase modes, the diversity and purposefulness of populations can be further enhanced, significantly improving the optimization's search ability and convergence speed for the optimal approximate solution.
\fi


==> key.tex <==
\begin{keywords}
Timing Optimization, Approximate Logic Synthesis, Double-chase Grey Wolf Optimizer, Gate Sizing
\end{keywords}

